Representation Learning for Point Cloud Understanding

With the rapid advancement of technology, 3D data acquisition and utilization have become increasingly prevalent across various fields, including computer vision, robotics, and geospatial analysis. 3D data, captured through methods such as 3D scanners, LiDARs, and RGB-D cameras, provides rich geometric, shape, and scale information. When combined with 2D images, 3D data offers machines a comprehensive understanding of their environment, benefiting applications like autonomous driving, robotics, remote sensing, and medical treatment. This dissertation focuses on three main areas: supervised representation learning for point cloud primitive segmentation, self-supervised learning methods, and transfer learning from 2D to 3D. Our approach, which integrates pre-trained 2D models to support 3D network training, significantly improves 3D understanding without merely transforming 2D data. Extensive experiments validate the effectiveness of our methods, showcasing their potential to advance point cloud representation learning by effectively integrating 2D knowledge.

==> README <==
                       utthesis2 2.0ame
                         February 2003

                     Ayman M. El-Khashab
                     ayman@austin.rr.com

This package provides a LaTeX 2e template and style file to produce a
master's or PhD. thesis that meets the requirements of the Graduate
School of The University of Texas at Austin.

The included files are based on utthesis.doc and utthesis.sty, which
were originally released by Dinesh Das in January 1995. They were
modified slightly by Bert Kay in 1996, by James A. Bednar in 1997, and
by Ayman M. El-Khashab in February 2003.  This February 2003 release
fixes several problematic interactions with other LaTeX packages, and
other bugs.  The details of the changes are attached to the end of
this file.

To get started, first make sure you can compile the included file
thesis.tex using your version of latex and/or pdflatex.  If that
works, then simply load thesis.tex into an editor and add your own
information as described in the comments in thesis.tex.

The PDF version of the thesis generated with pdflatex was verified to
meet the requirements of the graduate school as of February 2002 by
Lynn Renegar, Doctoral Evaluator.  Of course, it is crucial that you
actually check your own generated documents, both in PDF and printed
form, against the published guidelines of the graduate school.  The
requirements may have changed by the time you read this, and your
results may differ depending on your latex version, printer, degree
type, etc.


OPTIONAL PACKAGES

This template should work with any LaTeX 2e installation, and does not
require any external packages.  It should also work fine with such
packages, and I highly recommend those listed below.  If you want to
use these packages, first make sure that they are installed on your
system (e.g. "locate natbib.sty" in UNIX).  If they are not installed,
you can download them from CTAN, the Comprehensive TeX Archive
Network, and then put them in the same directory as you have placed
these files.  Then add \usepackage{<package-name>} to the preamble of
thesis.tex.  CTAN is mirrored at many locations worldwide, including
http://www.ctan.org/.


\usepackage{natbib}: provides support for author-year citations, as in
"Bednar (2002)", and better numeric citation handling.


\usepackage{hyperref}: when used with pdflatex, enables your table of
contents, citations, etc. to be hyperlinked.  The hyperlinks make it
much, much easier for your reader to navigate the PDF file.  For more
information about hyperref and pdflatex see
http://www.tug.org/applications/pdftex/.


\usepackage{tocbibind}: ensures that automatically-generated items
like the bibliography, list of figures, etc. show up in the table of
contents.  This is especially important with pdflatex/hyperref,
because tocbibind ensures that those entries are hyperlinked as well.
If you use tocbibind, you should remove the redundant \addcontentsline
line from thesis.tex.


\usepackage{graphics}: allows images to be included in the document.
Regular LaTeX supports only Encapsulated PostScript (EPS) images, but
PDFLaTeX supports JPEG, TIFF, PNG, and PDF formats, which makes
graphics inclusion much simpler.


DIFFERENCES FROM PREVIOUS RELEASES

The only differences introduced by JAB from the BKay 1996 release are
to remove the extra spacing on the title page, which causes problems
with multi-line titles, and to add the "Certification of approved
version" page with your committee members.  Differences introduced by
AME were to fix problems caused by old latex code (particularly of the
doublespace package) as well as problems with pdf bookmarks in the
abstract, TOC, list of figures/tables.  The detailed diffs follow,
and can be ignored entirely unless you are trying to integrate
multiple releases of these files.

Comparing the 1996 BKay release with the 2002 JAB release:

$ diff thesis.tex  ../utthesis-latex2e/utthesis.doc 
3,5c3
< %%% File: utthesis2.doc, version 2.0jab, February 2002
< %%%
< %%% Based on: utthesis.doc, version 2.0, January 1995
---
> %%% File: utthesis.doc, version 2.0, January 1995
29c27
< \usepackage {utthesis2}              %% Preamble.
---
> \usepackage {utthesis}               %% Preamble.
70,90d67
< % \renewcommand{\thesiscosupervisor}{}
<                                      %% Your PhD. thesis co-supervisor; if any.
<                                      %% Use mixed case and don't use any titles
<                                      %% or degrees. Uncomment if you
<                                      %% have a co-supervisor.
<                                      %% (Ignored for Master's)
< 
< \renewcommand{\thesiscommitteemembera}{}
< \renewcommand{\thesiscommitteememberb}{}
< \renewcommand{\thesiscommitteememberc}{}
< \renewcommand{\thesiscommitteememberd}{}
< % \renewcommand{\thesiscommitteemembere}{}
< % \renewcommand{\thesiscommitteememberf}{}
< % \renewcommand{\thesiscommitteememberg}{}
< % \renewcommand{\thesiscommitteememberh}{}
< % \renewcommand{\thesiscommitteememberi}{}
<                                      %% Define your other committee members here;
<                                      %% use mixed case and don't use any titles
<                                      %% or degrees.  Uncomment as many
<                                      %% as neccessary. (Ignored for Master's)
< 
141,142d117
< \thesiscertificationpage             %% Generate the PhD. certification page.
< 
145c120
< %\thesissignaturepage                %% Generate the Master's signature page.
---
> \thesissignaturepage                 %% Generate the signature page.
168,170d142
< 
< \addcontentsline {toc}{chapter}{Bibliography} 
<                                      %% Force Bibliography to appear in contents


$ diff utthesis2.sty   ../utthesis-latex2e/utthesis.sty 
3,5c3
< %%% File: utthesis2.sty, version 2.0jab, February 2002
< %%%
< %%% Based on: utthesis.sty, version 2.0, January 1995
---
> %%% File: utthesis.sty, version 2.0, January 1995
8d5
< %%%
12,19d8
< %%% Modified by James A. Bednar in March 1999.
< %%% My comments contain the string  ``JAB''.
< %%%
< %%% Extended by James A. Bednar in February 2002, based on 
< %%% portions of utdiss2-02.sty released on 29 November 2001
< %%% by Craig McCluskey (mccluskey@mail.utexas.edu).
< %%% His comments contain the string ``cwm''.
< %%%
181,183c170,171
< %% JAB
< \typeout{*************************************************************}
< \typeout{** UT Austin Thesis Style File, version 2.0jab, February 2002}
---
> \typeout{*************************************************************} 
> \typeout{** UT Austin Thesis Style File, version 2.0, January 1995    }
187d174
< \typeout{** Modified by Bert Kay and James A. Bednar                  }
214,223d200
< \newcommand{\thesiscosupervisor}{}
< \newcommand{\thesiscommitteemembera}{}
< \newcommand{\thesiscommitteememberb}{}
< \newcommand{\thesiscommitteememberc}{}
< \newcommand{\thesiscommitteememberd}{}
< \newcommand{\thesiscommitteemembere}{}
< \newcommand{\thesiscommitteememberf}{}
< \newcommand{\thesiscommitteememberg}{}
< \newcommand{\thesiscommitteememberh}{}
< \newcommand{\thesiscommitteememberi}{}
270,271d246
< 
< \newcommand{\@emptycommand}{} %% JAB  Used when testing if a command is defined but empty
333,334c308
<       % Commented-out by JAB 08Mar99 -- didn't leave any room for two-line title
<       %\strut \vfill    % Added BKay 17Oct96 -- title was too high on the page
---
>       \strut \vfill    % Added BKay 17Oct96 -- title was too high on the page
354,355c328
< %%% Command to generate old-style signature page, which as
< %%% of 2/2002 still seems to be used in Master's thesis.
---
> %%% Command to generate signature page.
381,457d353
< %%% Generates a signature line with the given name
< %%% Adapted from 26 Aug 2001 cwm by JAB
< %%%
< \newcommand{\thesissigline}[1]{%
<   \leftline{\hbox to 2.5in{}\hrulefill}
<   \endgraf
<   \vspace*{-18pt}
<   \leftline{\hbox to 2.53in{}{#1}}}
< 
< %%%
< %%% Generates signature lines for the committee
< %%% Adapted from 26 Aug 2001 cwm by JAB
< %%% Accepts up to two supervisors and eight other members
< %%%
< \newcommand{\thesiscertificationsignaturelines}{
<      \ifx\thesissupervisor\@emptycommand\relax\else
<         \thesissigline{\thesissupervisor, Supervisor}
<      \fi
<      \ifx\thesiscosupervisor\@emptycommand\relax\else
<         \thesissigline{\thesiscosupervisor, Supervisor}
<      \fi
<      \ifx\thesiscommitteemembera\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteemembera}
<      \fi
<      \ifx\thesiscommitteememberb\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberb}
<      \fi
<      \ifx\thesiscommitteememberc\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberc}
<      \fi
<      \ifx\thesiscommitteememberd\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberd}
<      \fi
<      \ifx\thesiscommitteemembere\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteemembere}
<      \fi
<      \ifx\thesiscommitteememberf\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberf}
<      \fi
<      \ifx\thesiscommitteememberg\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberg}
<      \fi
<      \ifx\thesiscommitteememberh\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberh}
<      \fi
<      \ifx\thesiscommitteememberi\@emptycommand\relax\else
<         \thesissigline{\thesiscommitteememberi}
<      \fi
<      }
< 
< %%%
< %%% Committee Certification Page
< %%%
< %%% Adapted from 26 Aug 2001 cwm by JAB
< %%%
< \newlength{\@tmplength}
< \newcommand{\thesiscertificationpage}{
<     \thispagestyle{empty}
<     \centerline{The Dissertation Committee for \thesisauthor}
<     \centerline{certifies that this is the approved version of the following dissertation:}
<     \vspace*{75pt}
<     \setlength\@tmplength\baselineskip
<     \baselineskip=16.5pt plus .5pt minus .2 pt
<     \baselineskip=28.5pt plus .5pt minus .2 pt
<     \begin{center}
<     \large\bf\@thesistitle
<     \end{center}
<     \vspace*{55pt}
<     \leftline{\hbox to 2.5in{}Committee:\hfill}
<     %\bigskip\medskip\smallskip
<     \bigskip
<     \thesiscertificationsignaturelines
<     \setlength\baselineskip\@tmplength
<     \clearpage}
< 
< 
< %%%
529,530c425
<        %% JAB: added other acks
<        of Texas at Austin, and extended by Bert Kay and James A. Bednar.
---
>        of Texas at Austin.


Comparing the 2002 JAB release with the 2003 AME release:

*** /tmp/utthesis2.sty.txt	Tue Feb 18 20:26:50 2003
--- utthesis2.sty	Tue Feb 18 21:00:53 2003
***************
*** 1,6 ****
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%
! %%% File: utthesis2.sty, version 2.0jab, February 2002
  %%%
  %%% Based on: utthesis.sty, version 2.0, January 1995
  %%% =============================================
--- 1,6 ----
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%
! %%% File: utthesis2.sty, version 2.0ame, February 2003
  %%%
  %%% Based on: utthesis.sty, version 2.0, January 1995
  %%% =============================================
***************
*** 17,22 ****
--- 17,28 ----
  %%% by Craig McCluskey (mccluskey@mail.utexas.edu).
  %%% His comments contain the string ``cwm''.
  %%%
+ %%% Modified by Ayman M. El-Khashab in February 2003, to fix
+ %%% problems caused by old latex code (particularly of the doublespace
+ %%% package) as well as problems with pdf bookmarks in the abstract,
+ %%% TOC, list of figures/tables.
+ %%% My comments contain the string ``AME''
+ %%%
  %%% This file is free and can be modified or distributed as long as
  %%% you meet the following conditions:
  %%%
***************
*** 178,191 ****
  %%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
! %% JAB
! \typeout{*************************************************************}
! \typeout{** UT Austin Thesis Style File, version 2.0jab, February 2002}
! \typeout{** Written by Dinesh Das                                     }
! \typeout{**            Dept. of Computer Sciences                     }
! \typeout{**            The University of Texas at Austin              }
! \typeout{** Modified by Bert Kay and James A. Bednar                  }
! \typeout{*************************************************************}
  
  %%%
  %%% Set up page layout parameters.
--- 184,197 ----
  %%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
! %% JAB/AME
! \typeout{****************************************************************}
! \typeout{** UT Austin Thesis Style File, version 2.0ame, February 2003   }
! \typeout{** Written by Dinesh Das                                        }
! \typeout{**            Dept. of Computer Sciences                        }
! \typeout{**            The University of Texas at Austin                 }
! \typeout{** Modified by Bert Kay, James A. Bednar, and Ayman El-Khashab  }
! \typeout{****************************************************************}
  
  %%%
  %%% Set up page layout parameters.
***************
*** 271,279 ****
  \newcommand{\@emptycommand}{} %% JAB  Used when testing if a command is defined but empty
  \newcommand{\@defaultbaselinestretch}{1.5}
  \newcommand{\@base}[1]{\renewcommand{\baselinestretch}{#1}}
! \newcommand{\singlespace}{\renewcommand{\@defaultbaselinestretch}{1.1}}
! \newcommand{\oneandhalfspace}{\renewcommand{\@defaultbaselinestretch}{1.5}}
! \newcommand{\doublespace}{\renewcommand{\@defaultbaselinestretch}{1.7}}
  \newcommand{\@thesistitle}{\textbf{\thesistitletypesize \thesistitle}}
  \newcommand{\@thesisapprovedby}%
      {\textbf{\thesisapprovedbytypesize \thesisapprovedby}}
--- 277,288 ----
  \newcommand{\@emptycommand}{} %% JAB  Used when testing if a command is defined but empty
  \newcommand{\@defaultbaselinestretch}{1.5}
  \newcommand{\@base}[1]{\renewcommand{\baselinestretch}{#1}}
! 
! %%% AME: Changed to use setspace environments
! \newcommand{\singlespace}{singlespacing}
! \newcommand{\oneandhalfspace}{onehalfspacing}
! \newcommand{\doublespace}{\doublespacing}
! 
  \newcommand{\@thesistitle}{\textbf{\thesistitletypesize \thesistitle}}
  \newcommand{\@thesisapprovedby}%
      {\textbf{\thesisapprovedbytypesize \thesisapprovedby}}
***************
*** 458,464 ****
  %%% Environment to generate abstract page.
  %%%
  \newenvironment{thesisabstract}
!     {\addcontentsline{toc}{chapter}{Abstract}
       \vspace*{0mm}
       \begin{center}
         \setlength{\unitlength}{1mm}
--- 467,474 ----
  %%% Environment to generate abstract page.
  %%%
  \newenvironment{thesisabstract}
!     {\chapter*{}
!      \addcontentsline{toc}{chapter}{Abstract}
       \vspace*{0mm}
       \begin{center}
         \setlength{\unitlength}{1mm}
***************
*** 526,534 ****
         trademark of the American Mathematical Society.  The macros used in
         formatting this \lowercase\expandafter{\thesistype} were written
         by Dinesh Das, Department of Computer Sciences, The University
!        %% JAB: added other acks
!        of Texas at Austin, and extended by Bert Kay and James A. Bednar.
!     } by \thesistypist.}
  
  \newcommand{\@chapteralignment}{\centering}
  \renewcommand{\chapter}{\clearpage
--- 536,544 ----
         trademark of the American Mathematical Society.  The macros used in
         formatting this \lowercase\expandafter{\thesistype} were written
         by Dinesh Das, Department of Computer Sciences, The University
!        %% AME: added other acks
!        of Texas at Austin, and extended by Bert Kay, James A. Bednar, and Ayman El-Khashab.
! 	  } by \thesistypist.}
  
  \newcommand{\@chapteralignment}{\centering}
  \renewcommand{\chapter}{\clearpage
***************
*** 642,647 ****
--- 652,658 ----
  %%% Command from report.cls, (c) LaTeX3 Project.
  %%%
  \renewcommand\listoftables{%
+     \clearpage  %%% AME 
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
***************
*** 654,659 ****
--- 665,671 ----
      \if@restonecol\twocolumn\fi
      }
  \renewcommand\listoffigures{%
+     \clearpage  %%% AME 
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
***************
*** 748,821 ****
  \def\timestamp{\thesistime, \thesisdayofweek, \thesisdate}
  
  %%%
! %%% Commands for spacing.  Some parts from spacing.sty by Stephen Page.
  %%% 
! \ifx\undefined\selectfont
! \def\@setsize#1#2#3#4{\@nomath#1
!    \let\@currsize#1\baselineskip
!    #2\baselineskip\baselinestretch\baselineskip
!    \parskip\baselinestretch\parskip
!    \setbox\strutbox\hbox{\vrule height.7\baselineskip
!       depth.3\baselineskip width\z@}
!    \normalbaselineskip\baselineskip#3#4}
! \else
! \def\@newbaseline{%
!     \ifx\undefined\setnew@baselineskip
!       \baselineskip\f@baselineskip\relax
!     \else
!       \setnew@baselineskip
!     \fi
!     \baselineskip\baselinestretch\baselineskip
!     \setbox\strutbox\hbox{\vrule\@height.7\baselineskip
!     \@depth.3\baselineskip \@width\z@}%
!     \normalbaselineskip\baselineskip}
! \fi
! %%%
! %%% Reset baselinestretch within footnotes and floats. Originally stolen
! %%% from Stanford thesis style.
! %%%
! \def\@xfloat#1[#2]{\ifhmode \@bsphack\@floatpenalty -\@Mii\else
!    \@floatpenalty-\@Miii\fi\def\@captype{#1}\ifinner
!       \@parmoderr\@floatpenalty\z@
!     \else\@next\@currbox\@freelist{\@tempcnta\csname ftype@#1\endcsname
!        \multiply\@tempcnta\@xxxii\advance\@tempcnta\sixt@@n
!        \@tfor \@tempa :=#2\do
!                         {\if\@tempa h\advance\@tempcnta \@ne\fi
!                          \if\@tempa t\advance\@tempcnta \tw@\fi
!                          \if\@tempa b\advance\@tempcnta 4\relax\fi
!                          \if\@tempa p\advance\@tempcnta 8\relax\fi
!          }\global\count\@currbox\@tempcnta}\@fltovf\fi
!     \global\setbox\@currbox\vbox\bgroup 
!     \def\baselinestretch{1}
!     \ifx\undefined\selectfont
!     \small\normalsize
!     \else
!     \@newbaseline
!     \fi
!     \boxmaxdepth\z@
!     \hsize\columnwidth \@parboxrestore}
! \long\def\@footnotetext#1{\insert\footins{\def\baselinestretch{1}\footnotesize
!     \interlinepenalty\interfootnotelinepenalty 
      \splittopskip\footnotesep
      \splitmaxdepth \dp\strutbox \floatingpenalty \@MM
!     \hsize\columnwidth \@parboxrestore
!    \edef\@currentlabel{\csname p@footnote\endcsname\@thefnmark}\@makefntext
!     {\rule{\z@}{\footnotesep}\ignorespaces
!       #1\strut}}}
! %%%
! %%% Stolen from MIT.
! %%%
! \def\spacing#1{\par%
!  \begingroup
!  \def\baselinestretch{#1}
!  \ifx\undefined\selectfont
!  \ifx\@currsize\normalsize\@normalsize\else\@currsize\fi
!  \else
!  \@newbaseline
!  \fi}
! \def\endspacing{\par
!  \vskip \parskip
!  \vskip \baselineskip
!  \endgroup
!  \vskip -\parskip
!  \vskip -\baselineskip}
--- 760,894 ----
  \def\timestamp{\thesistime, \thesisdayofweek, \thesisdate}
  
  %%%
! %%% Spacing commands
! %%%
! %%% Most from setspace.sty by Geoffrey Tobin 
  %%% 
! %%%
! 
! \newcommand{\setstretch}[1]{%   %%% AME setup to use setspace macros
!   \def\baselinestretch{#1}%
!   \@currsize
! }
! 
! \newcommand{\SetSinglespace}[1]{%
!   \def\setspace@singlespace{#1}%
! }
! 
! \SetSinglespace{1}
! 
! \newcommand{\singlespacing}{%
!   \setstretch {\setspace@singlespace}%  normally 1
!   \vskip \baselineskip  % Correction for coming into singlespace
! }
! 
! \newcommand{\onehalfspacing}{%
!   \setstretch{1.25}%  default
!   \ifcase \@ptsize \relax % 10pt
!     \setstretch {1.25}%
!   \or % 11pt
!     \setstretch {1.213}%
!   \or % 12pt
!     \setstretch {1.241}%
!   \fi
! }
! 
! \newcommand{\doublespacing}{%
!   \setstretch {1.667}%  default
!   \ifcase \@ptsize \relax % 10pt
!     \setstretch {1.667}%
!   \or % 11pt
!     \setstretch {1.618}%
!   \or % 12pt
!     \setstretch {1.655}%
!   \fi
! }
! 
! 
! %%%
! %%% AME:  This is to correct spacing after the tabular env.
! %%% according to the maintainers of setspace
! %%%
! 
! \def\@setsize#1#2#3#4{%
!   % Modified 1993.04.07--GDG per KPC
!   \@nomath#1%
!   \let\@currsize#1%
!   \baselineskip #2%
!   \baselineskip \baselinestretch\baselineskip
!   \parskip \baselinestretch\parskip
!   \setbox\strutbox \hbox{%
!     \vrule height.7\baselineskip
!            depth.3\baselineskip
!            width\z@}%
!   \skip\footins \baselinestretch\skip\footins
!   \normalbaselineskip\baselineskip#3#4}
! 
! 
! %%%
! %%% Adjust the spacing for floats (reset to single space)
! %%%
! 
! \let\latex@xfloat=\@xfloat
! \def\@xfloat #1[#2]{%
!   \latex@xfloat #1[#2]%
!   \def\baselinestretch{\setspace@singlespace}%
!   \normalsize
! }
! 
! 
! %%% 
! %%% Footnotes, AME, did not bring over minipage footnotes
! %%% 
! 
! \long\def\@footnotetext#1{%
!   \insert\footins{%
!     \def\baselinestretch {\setspace@singlespace}%
!     \reset@font\footnotesize
!     \interlinepenalty\interfootnotelinepenalty
      \splittopskip\footnotesep
      \splitmaxdepth \dp\strutbox \floatingpenalty \@MM
!     \hsize\columnwidth
!     \@parboxrestore
!     \protected@edef\@currentlabel{%
!       \csname p@footnote\endcsname\@thefnmark
!     }%
!     \color@begingroup
!       \@makefntext{%
!         \rule\z@\footnotesep\ignorespaces#1\@finalstrut\strutbox}%
!     \color@endgroup}}
! 
! %%%
! %%% AME Fix the spacing around display math
! %%%
! \newcommand{\displayskipstretch}{\baselinestretch}
! \newcommand{\setdisplayskipstretch}[1]{\renewcommand{\displayskipstretch}{#1}}
! \everydisplay\expandafter{%
!   \the\everydisplay
!   \abovedisplayskip \displayskipstretch\abovedisplayskip
!   \belowdisplayskip \displayskipstretch\belowdisplayskip
!   \abovedisplayshortskip \displayskipstretch\abovedisplayshortskip
!   \belowdisplayshortskip \displayskipstretch\belowdisplayshortskip
! }
! 
! %%%
! %%% AME Modified to use the setspace style commands
! %%% 
! 
! \newcommand{\restore@spacing}{%
!     \par
!     \vskip \parskip
!     \vskip \baselineskip
!   \endgroup
!   \vskip -\parskip
!   \vskip -\baselineskip
! }
! 
! \newenvironment{spacing}[1]{%
!   \par
!   \begingroup             
!   \setstretch {#1}%
! }{ 
!   \restore@spacing
! }
! 


==> chapters/IAE/figures_tex/analysis.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.8\textwidth]{CVPR_2023/figures/compare_cvpr2023.pdf}
\caption{\small{\textbf{Comparison between explicit and implicit auto-encoder.} \textbf{Left:} T-SNE visualization for encoder features of EAE(blue) and IAE(orange). The encoder features of IAE is tighter than EAE.
\textbf{Right:} `implicit' denotes IAE pretrained with sdf label generated by water-tight mesh. `implicit w/o mesh' denotes IAE pretrained with udf label generated by the original point cloud. 
%`Acc Diff' denotes the accuracy difference between two models on ModelNet40 Linear. 
`gap' denotes the accuracy difference between `implicit' and `explicit'. When increasing the input resolution, the gap between explicit and implicit models decreases.\protect\footnotemark. }}
    \label{fig:analysis}
    %%\vspace{-30pt}
\end{figure*}



==> chapters/IAE/figures_tex/completion.tex <==
\begin{figure}[t]
\begin{minipage}[b]{.46\linewidth}
    \centering
    \begin{tabular}{l|lc}
    \toprule
    Decoder & Method & SUN RGB-D \\
        \midrule
        \multirow{3}{*}{Explicit} &  FoldingNet~\cite{yang2018foldingnet} & 58.2 \\
        & OcCo~\cite{wang2020unsupervised} & 58.4  \\
        & SnowflakeNet~\cite{xiang2021snowflakenet} & 58.1 \\
        \midrule
        Implicit & Conv-OccNet~\cite{peng2020convolutional} &  \textbf{60.4} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\textbf{Comparison between explicit approaches and our model} on real data completion task. Our model built upon convolutional occupancy network shows consistent improvements.}
    \label{tab:complete_comp}
\end{minipage}\hspace{.02\lin ewidth}
\begin{minipage}[b]{.5\linewidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/completion.png}
    \caption{\textbf{Qualitative completion results on ScanNet.}  We show the results of SnowflakeNet~\cite{xiang2021snowflakenet} and our model.}
    \label{fig:complete}
\end{minipage}
%\vspace{-15pt}
\end{figure}

==> chapters/IAE/figures_tex/teaser_v2.tex <==
\begin{figure}[t]
    \centering
    %\vspace{+0.1in}
    \includegraphics[width=\columnwidth]{figures/fig1_update_2.pdf}
    %\vspace{+0.1in}
    \caption{\small{\textbf{Explicit Autoencoder versus Implicit Autoencoder (Ours)}. Given one shape with $N$ samples, for the traditional explicit autoencoder, the model is forced to reconstruct the input one-to-one. For the implicit autoencoder, the reconstruction targets are the same.}}
    \label{fig:teaser}
    \vspace{-10pt}
\end{figure}

==> chapters/IAE/tables/cls.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|cc}
        \toprule
        \textbf{Method} & \textbf{\#points} & \textbf{Acc. (\%)} \\
        \midrule
        PointNet~\cite{qi2017pointnet++} & 1k & 89.2 \\
        PointNet++~\cite{qi2017pointnet} & 1k &  90.7 \\
        PointCNN~\cite{li2018pointcnn} & 1k & 92.2 \\
        KPConv~\cite{thomas2019kpconv} & 1k & 92.9 \\
        PointTransform~\cite{zhao2021point} & 1k & 93.7 \\
        PointNeXt~\cite{qian2022pointnext} & 1k & 93.2 \\
        PointMLP~\cite{ma2022rethinking} & 1k & 94.1 \\
        \midrule
        PointViT~\cite{yu2021point} & 1k & 91.4 \\
        $\text{[S]}$ Point-BERT~\cite{yu2021point} & 1K & 93.2 \\
        $\text{[S]}$Point-MAE~\cite{pang2022masked} & 1k & 93.8 \\
        $\text{[S]}$Point-MAE~\cite{pang2022masked} & 8k & \underline{94.0} \\
        DGCNN~\cite{wang2019dynamic} &  1k & 92.9 \\
        $\text{[S]}$FoldingNet~\cite{yang2018foldingnet}* & 1k & 93.1 \\
        $\text{[S]}$STRL~\cite{huang2021spatio}* & 1k & 93.1 \\
        $\text{[S]}$OcCo~\cite{wang2020unsupervised}* & 1k & 93.0 \\
        \rowcolor{gray!20} $\text{[S]}$IAE w/o mesh* & 1k & 94.0\\
        \rowcolor{gray!20} $\text{[S]}$IAE* & 1k & \textbf{94.2} \textcolor[rgb]{0,0.6,0}{(+1.2)} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Shape classification fine-tuned results on ModelNet40.} Supervised methods train from scratch. Self-supervised methods(denoted by [S]) use the pre-trained models as the initial weight for supervised fine-tuning. `$\#$points' denotes number of input points. * methods use the same DGCNN encoder backbone. \textcolor[rgb]{0,0.6,0}{green} number shows the absolute improvement under the same backbone.}}
    \label{tab:mn40_ft}
\vspace{-0.1in}
\end{table}

==> chapters/IAE/tables/detection_seg.tex <==
\begin{table*}[t]
\small
\begin{minipage}[t]{.55\linewidth}
    \centering
   \setlength\tabcolsep{10pt}% 调整列间距
    \begin{tabular}{lcccc}
        \toprule
     Method  & \multicolumn{2}{c}{ScanNet} & \multicolumn{2}{c}{SUN RGB-D} \\
        \cmidrule(lr){2-3}   \cmidrule(lr){4-5}  & $\text{AP}_{25}$ & $\text{AP}_{50}$ & $\text{AP}_{25}$ & $\text{AP}_{50}$ \\
        \midrule
        VoteNet~\cite{qi2019deep}  &  58.6 & 33.5 & 57.7 & 32.9 \\
        3D-MPA~\cite{engelmann20203d} & 64.2 & 49.2 & - & - \\
        MLCVNet~\cite{xie2020mlcvnet} & 64.5 & 41.4 & 59.8 & - \\
        %H3DNet~\cite{zhang2020h3dnet} & 67.2 & 48.1 & 60.1 & 39.0 \\
        BRNet~\cite{cheng2021back} & 66.1 & 50.9 & 61.1 & 43.7 \\
        3DETR~\cite{misra2021end} & 65.0 & 47.0 & 59.1 & 32.7 \\
        GroupFree~\cite{liu2021group} & 69.1 & 52.8 & 63.0 & 45.2 \\
        FCAF3D~\cite{rukhovich2021fcaf3d} & 71.5 & 57.3 & 64.2 & 48.9 \\
        CAGroup3D~\cite{wang2022cagroup3d} & 75.1 & 61.3 & 66.8 & 50.2 \\
        \midrule
        %OcCo\cite{wang2020unsupervised} & 59.8 & 37.9 & 59.6 & 34.8 \\
        STRL~\cite{huang2021spatio} & 59.5 & 38.4 & 58.2 & 35.0 \\
        RandomRooms~\cite{rao2021randomrooms} & 61.3 & 36.2 & 59.2 & 35.4 \\
        PointContrast~\cite{xie2020pointcontrast} & 59.2 & 38.0 & 57.5 & 34.8 \\
        DepthContrast\protect\footnotemark~\cite{zhang2021self} & 62.1 & 39.1 & 60.4 & 35.4 \\
        Point-M2AE~\cite{zhang2022point} & 66.3 & 48.3 & - & - \\
        %DepthContrast($3\times$; \text{both}) & 64.0 & 42.9 \\
        IAE (VoteNet) & 61.5 & 39.8 & 60.4 & 36.0 \\
        IAE (CAGroup3D) & \textbf{76.1} & \textbf{62.0} & \textbf{67.6} & \textbf{51.3}\\
        \bottomrule
    \end{tabular}
    \caption{\small{\textbf{3D Object Detection Results.} We fine-tune our pre-trained model on ScanNetV2~\cite{dai2017scannet} and SUN-RGBD~\cite{song2015sun} validation sets using VoteNet~\cite{qi2019deep} and CAGroup3D~\cite{wang2022cagroup3d}. We show mean Average Precision~(mAP) across all semantic classes with 3D IoU thresholds of 0.25 and 0.5. Methods in the second section denote self-supervised methods.}}
    \label{tab:detection}
\end{minipage}\hspace{.02\linewidth}
\begin{minipage}[t]{.4\linewidth}
 \setlength\tabcolsep{15pt}
    \begin{tabular}{lcc}
        \toprule
        Method & \multicolumn{2}{c}{S3DIS 6-Fold} \\
        \cmidrule(lr){2-3} & OA & mIoU \\
        \midrule
        PointNet~\cite{qi2017pointnet} & 78.5 & 47.6 \\
        PointCNN~\cite{li2018pointcnn} & 88.1 & 65.4 \\
        DGCNN~\cite{wang2019dynamic} & 84.1 & 56.1 \\
        DeepGCN~\cite{} & 85.9 & 60.0 \\
        KPConv~\cite{thomas2019kpconv} & - & 70.6 \\
        RandLA-Net~\cite{hu2020randla} & 88.0 & 70.0 \\
        BAAF-Net~\cite{qiu2021semantic} & 88.0 & 70.0 \\
        PointTransformer~\cite{zhao2021point} & 90.2 & 73.5 \\
        CBL~\cite{tang2022contrastive} & 89.6 & 73.1 \\
        PointNeXt~\cite{qian2022pointnext} & 90.3 & 74.9 \\
        \midrule
        Jigsaw~\cite{sauder2019self} & 84.4 & 56.6 \\
        OcCo~\cite{wang2020unsupervised} & 85.1 & 58.5 \\
        STRL~\cite{huang2021spatio} & 84.2 & 57.1 \\ 
        IAE (DGCNN) & 85.9 & 60.7 \\
        IAE (PointNeXt) & \textbf{90.8} & \textbf{75.3} \\
        
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Semantic Segmentation Results on S3DIS~\cite{armeni20163d} 6-Fold.} We show Overall Accuracy (OA) and mean Intersection over Union~(mIoU) across six folds.}}
    \label{tab:semseg}
\end{minipage}
\vspace{-4mm}
\end{table*}

==> chapters/IAE/tables/diff_aug_3.tex <==
\begin{table}[t]
    \centering
   %\setlength\tabcolsep{6pt}% 调整列间距
   %\renewcommand\arraystretch{1.1}
   %\vspace{-15pt}
    \begin{tabular}{c|ccccc}
        \toprule
        Aug & scratch & cr=0 & cr=20\% & cr=50\%& cr=70\% \\
        \hline
        SUN & 57.7 & 60.0 & 60.2 & \textbf{60.4} & 59.8 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Different setting of scene data augmentation.} `cr' denotes max cropping ratio. `scratch' means training from scratch.}
    \label{tab:data_aug}
\end{table}

==> chapters/IAE/tables/svm.tex <==
\begin{table}[h]
    %\resizebox{\textwidth}{20mm}
    \centering
    \setlength\tabcolsep{25pt}
    \begin{tabular}{l|c}
        \toprule
        \textbf{Method} & \textbf{Acc. (\%)} \\
        \midrule
        %Random &  60.2\% \\
        3D-GAN~\cite{wu2016learning}  & 83.3 \\
        Latent-GAN~\cite{achlioptas2018learning} & 85.7 \\
        SO-Net~\cite{li2018so} & 87.3 \\
        MAP-VAE~\cite{han2019multi} & 88.4 \\
        Point-BERT~\cite{yu2021point} & 87.4 \\
        Point-MAE~\cite{pang2022masked} & 88.5 \\
        \midrule
        Jigsaw~\cite{sauder2019self}$^*$ & 84.1 \\
        FoldingNet~\cite{yang2018foldingnet}$^*$ & 90.1 \\
        Orientation~\cite{poursaeed2020self}$^*$ & 90.7 \\
        STRL~\cite{huang2021spatio}$^*$ & 90.9 \\
        OcCo~\cite{wang2020unsupervised}$^*$ & 89.7 \\
        CrossPoint~\cite{afham2022crosspoint} $^*$ & 91.2 \\
        \rowcolor{gray!20} IAE w/o mesh$^*$ & 91.7 \\
        \rowcolor{gray!20} IAE$^*$ & \textbf{92.1} \textcolor[rgb]{0,0.6,0}{(+0.9)} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Linear evaluation for shape classification on ModelNet40}. For fair comparisons, different $^*$ methods use the same DGCNN encoder backbone. \textcolor[rgb]{0,0.6,0}{green} number shows the absolute improvement.}}
    \label{tab:mn40}
%\vspace{-0.1in}
\end{table}

==> chapters/MVNet/algorithm/algorithm.tex <==
\begin{algorithm}
\caption{General framework of MVNet}
\begin{algorithmic}[1]
\State \textbf{Input:} RGB-D scan pairs with camera parameters $S = \{(I_1^{i}, D_1^{i}), (I_2^{i}, D_2^{i}), K^{i}, E_1^{i}, E_2^{i}\}$, feature encoding network $\mathcal{F}_e$, 2D knowledge transfer module $\mathcal{F}_{2d}$, multi-view consistency module $\mathcal{F}_m$.
\State \textbf{Ouput:} Pre-trained weights of feature encoding network $\mathcal{F}_e$

\For{$\{(I_1, D_1), (I_2, D_2), K, E_1, E_2\}$ \textbf{in} RGB-D scan pairs}
\State - Project $(I_1, D_1), (I_2, D_2)$ into 3D point cloud $P$ via camera parameters $K, E_1, E_2$.
\State - Extract per-point feature volume: $F_P = \mathcal{F}_e(P)$.
\State - Project the feature volume back onto the original views to generate 2D feature maps $F_1, F_2$
\State - Employ 2D knowledge transfer module with square $L_2$ loss: $\mathcal{L}_{2d} = \mathcal{F}_{2d}(I_i, F_i)$
\State - Employ multi-view consistency module with the correspondence loss: $\mathcal{L}_{m} = \mathcal{F}_m(F_1, F_2)$
\State - Compute the total loss $\mathcal{L} = \mathcal{L}_{2d} + \lambda \mathcal{L}_m$.
\State - Backprop: to update $\mathcal{F}_e, \mathcal{F}_{2d}, \mathcal{F}_m$ with loss $\mathcal{L}$.
\EndFor
\end{algorithmic}
\label{alg:mvnet}
\end{algorithm}

==> chapters/MVNet/figures/supp_cotr_2.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{images/supp_cotr.pdf}
    \end{center}
    \caption{\textbf{Qualitative results of multi-view consistency module prediction.} Each element consists of two different view images. The query points and prediction points are visualized using the blue dot, and they are connected by the green line.}
    \label{Fig:supp_cotr}
\end{figure}

==> chapters/MVNet/figures/supp_eff.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{images/label_eff.pdf}
    \end{center}
    \caption{\textbf{Illustration of Label efficiency training.} Our model is pre-trained on ScanNet and subsequently fine-tuned separately on both ScanNet and SUN RGBD. We take VoteNet as network architecture. During this fine-tuning process, we employ varying percentages of labeled training data. Demonstrating its efficacy, our pre-training model not only surpasses the performance of models trained from scratch but also achieves comparable results utilizing only 60\% of the labeled data.}
    \label{fig:eff}
\end{figure}

==> chapters/MVNet/figures/supp_qual.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=\linewidth]{images/visualize-3.pdf}
    \end{center}
    \caption{\textbf{Qualitative results on S3DIS semantic segmentation task.} We compare our method with the second-best approach, SceneContext~\citep{hou2021exploring}.}
    \label{Fig:srnet}
\end{figure}

==> chapters/MVNet/figures/supp_qual_2.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=\linewidth]{images/visualize_4.pdf}
    \end{center}
    \caption{\textbf{More qualitative results on S3DIS semantic segmentation task.} We compare our method with the second-best approach, SceneContext~\citep{hou2021exploring}.}
    \label{Fig:srnet}
\end{figure}

==> chapters/MVNet/figures/supp_radar_chart.tex <==
\begin{figure}[h]
    \centering   
    \includegraphics[width=0.7\linewidth]{images/radar_chart_multi.pdf}
    %\caption{Our model (blue) achieves state-of-the-art performance across a broad range of tasks at both the scene and shape levels. The distance to the origin indicates the task result.}
    \label{fig:radar}
\end{figure}

==> chapters/MVNet/figures/supp_srnet.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{images/sr-unet.pdf}
    \end{center}
    \caption{\textbf{Feature encoding network details.}}
    \label{Fig:srnet}
\end{figure}

==> chapters/MVNet/tables/detection.tex <==
\begin{table*}[t]
\centering
    \caption{\small{\textbf{3D Object Detection Results.} We fine-tune our pre-trained model on ScanNetV2~\cite{dai2017scannet} and SUN-RGBD~\cite{song2015sun} validation sets using VoteNet~\cite{qi2019deep} and CAGroup3D~\cite{wang2022cagroup3d}. We show mean Average Precision~(mAP) across all semantic classes with 3D IoU thresholds of 0.25 and 0.5. Methods in the second section denote self-supervised methods.}}
    \label{tab:detection}
   \setlength\tabcolsep{9pt}% 调整列间距
    \begin{tabular}{lcccccc}
        \toprule
     \multirow{2}{*}{Method} & \multirow{2}{*}{SSL} & \multicolumn{2}{c}{ScanNet} & \multicolumn{2}{c}{SUN RGB-D} \\
        \cmidrule(lr){3-4}   \cmidrule(lr){5-6}  & 
       &  mAP@0.25 & mAP@0.5 & mAP@0.25 & mAP@0.5 \\
        \midrule
        VoteNet~\cite{qi2019deep} & - &  58.6 & 33.5 & 57.7 & 32.9 \\
        3D-MPA~\cite{engelmann20203d}& - & 64.2 & 49.2 & - & - \\
        MLCVNet~\cite{xie2020mlcvnet}& - & 64.5 & 41.4 & 59.8 & - \\
        %H3DNet~\cite{zhang2020h3dnet} & 67.2 & 48.1 & 60.1 & 39.0 \\
        BRNet~\cite{cheng2021back}& - & 66.1 & 50.9 & 61.1 & 43.7 \\
        3DETR~\cite{misra2021end}& - & 65.0 & 47.0 & 59.1 & 32.7 \\
        GroupFree~\cite{liu2021group}& - & 69.1 & 52.8 & 63.0 & 45.2 \\
        FCAF3D~\cite{rukhovich2021fcaf3d} & - & 71.5 & 57.3 & 64.2 & 48.9 \\
        CAGroup3D~\cite{wang2022cagroup3d} & - & 75.1 & 61.3 & 66.8 & 50.2 \\
        \midrule
        %OcCo\cite{wang2020unsupervised} & 59.8 & 37.9 & 59.6 & 34.8 \\
        STRL~\cite{huang2021spatio}& \checkmark & 59.5 & 38.4 & 58.2 & 35.0 \\
        RandomRooms~\cite{rao2021randomrooms}& \checkmark & 61.3 & 36.2 & 59.2 & 35.4 \\
        PointContrast~\cite{xie2020pointcontrast}& \checkmark & 59.2 & 38.0 & 57.5 & 34.8 \\
        DepthContrast~\cite{zhang2021self}& \checkmark & 62.1 & 39.1 & 60.4 & 35.4 \\
        Point-M2AE~\cite{zhang2022point}& \checkmark & 66.3 & 48.3 & - & - \\
        %DepthContrast($3\times$; \text{both}) & 64.0 & 42.9 \\
        \rowcolor{gray!20} MVNet + VoteNet & \checkmark & - & - & - & - \\
        \rowcolor{gray!20} MVNet + CAGroup3D & \checkmark & - & - & - & -\\
        \bottomrule
    \end{tabular}
\vspace{-4mm}
\end{table*}

==> chapters/MVNet/tables/detection_spv.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{9pt}% 调整列间距
\begin{tabular}{lccccc}
    \toprule
     \multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanNet} & \multicolumn{2}{c}{SUN RGB-D} \\
        \cmidrule(lr){2-3}   \cmidrule(lr){4-5}  & 
        mAP@0.25 & mAP@0.5 & mAP@0.25 & mAP@0.5 \\
        \midrule
        VoteNet~\cite{qi2019deep} & 58.6 & 33.5 & 57.7 & 32.9 \\
        3D-MPA~\cite{engelmann20203d}& 64.2 & 49.2 & - & - \\
        HGNet~\cite{chen2020hierarchical} & 61.3 & 34.4 & 61.6 & - \\
        MLCVNet~\cite{xie2020mlcvnet}& 64.5 & 41.4 & 59.8 & - \\
        %GSDN~\cite{gwak2020generative} & 62.8 & 34.8 & - & - \\
        H3DNet~\cite{zhang2020h3dnet} & 67.2 & 48.1 & 60.1 & 39.0 \\
        BRNet~\cite{cheng2021back}& 66.1 & 50.9 & 61.1 & 43.7 \\
        3DETR~\cite{misra2021end}& 65.0 & 47.0 & 59.1 & 32.7 \\
        VENet~\cite{xie2021venet} & 67.7 & - & 62.5 & 39.2 \\
        GroupFree~\cite{liu2021group}& 69.1 & 52.8 & 63.0 & 45.2 \\
        RGBNet~\cite{wang2022rbgnet} & 70.6 & 55.2 & 64.1 & 47.2 \\
        HyperDet3D~\cite{zheng2022hyperdet3d} & 70.9 & 57.2 & 63.5 & 47.3 \\
        FCAF3D~\cite{rukhovich2021fcaf3d} & 71.5 & 57.3 & 64.2 & 48.9 \\
        CAGroup3D~\cite{wang2022cagroup3d} & 75.1 & 61.3 & 66.8 & 50.2 \\
        \rowcolor{gray!20} MVNet + CAGroup3D & \textbf{75.5}\small{±0.3} & \textbf{61.8}\small{±0.3} & \textbf{67.2}\small{±0.2} & \textbf{51.1}\small{±0.3}\\
        \bottomrule
    \end{tabular}
\caption{\small{\textbf{Comparison of 3D object detection results with supervised methods.} We fine-tune our pre-trained model on ScanNetV2~\cite{dai2017scannet} and SUN-RGBD~\cite{song2015sun} datasets using CAGroup3D~\cite{wang2022cagroup3d}.}}
\label{tab:detection_spv}
\vspace{-4mm}
\end{table*}

==> chapters/MVNet/tables/loss_ablation.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation study on loss design.}
    \label{tab:ablation}
   \setlength\tabcolsep{6pt}% 调整列间距
    \begin{tabular}{cc|c}
        \toprule
        $\mathcal{L}_{2d}$ &$\mathcal{L}_m$ & ScanNet \\
        \midrule
        - & - & \\
         $\surd$ & - & \\
        -& $\surd$ &  \\
        $\surd$ & $\surd$ & \\
        \bottomrule
    \end{tabular}
\end{table}

==> chapters/MVNet/tables/seg_det.tex <==
\begin{table*}[h]
\centering
\footnotesize
\setlength\tabcolsep{4pt}
\begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{Method} & \multicolumn{5}{c}{Semantic Segmentation} & \multicolumn{4}{c}{3D Object Detection} \\
    & \multicolumn{3}{c}{S3DIS Area 5} & \multicolumn{3}{c}{S3DIS 6-Fold} & ScanNet \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8} & OA & mIoU & OA & mIoU & mIoU & \\
    \midrule
    Jigsaw & 82.8 & - & 52.1 & 84.4 & - & 56.6& - \\
    OcCo & 85.9 & - & 55.4 & 85.1 & - & 58.5 & - \\
    STRL & -  & - & - & 84.2 & - & 57.1 & -\\ 
    PointContrast  &  - & 77.0 & 70.9 & - & - & - & 74.1 \\ 
    DepthContrast & -  & - & 70.6 & - & - & - & 71.2\\ 
    SceneContext &  - & - & 72.2 & - & - & - & 73.8 \\ 
    \rowcolor{gray!20} MVNet & \textbf{91.7}(91.6) & \textbf{79.5}(79.3) & \textbf{73.6}(73.3) & \textbf{91.8}(91.7) & \textbf{86.3}(86.2) & \textbf{78.3}(78.1) & \textbf{75.6}(75.2)\\
    
    %\rowcolor{gray!20}\textit{ Improvement} & \textcolor[rgb]{0,0.6,0}{+2.6} & \textcolor[rgb]{0,0.6,0}{+4.1} & \textcolor[rgb]{0,0.6,0}{+5.4} & \textcolor[rgb]{0,0.6,0}{+1.6} & \textcolor[rgb]{0,0.6,0}{+4.2} & \textcolor[rgb]{0,0.6,0}{+4.7} & \textcolor[rgb]{0,0.6,0}{+3.4}\\
    \bottomrule
\end{tabular}
\caption{\small{\textbf{Semantic segmentation results on S3DIS (evaluation by 6-Fold or in Area 5) and ScanNet V2.} We show Overall Accuracy (OA), mean Accuracy (mAcc), and mean Intersection over Union~(mIoU). Methods in the second section are self-supervised pre-training approaches. MVNet shows the average results of 3 runs.}}
\label{tab:semseg}
\end{table*}

==> chapters/MVNet/tables/segmentation_3.tex <==
\begin{table*}[h]
\centering
\footnotesize
\setlength\tabcolsep{4pt}
\begin{tabular}{llllllll}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{S3DIS Area 5} & \multicolumn{3}{c}{S3DIS 6-Fold} & ScanNet \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8} & OA & mAcc & mIoU & OA & mAcc & mIoU & mIoU \\
    \midrule
    %PointNet & 53.5 & 49.0 & 41.1 & 78.5 & 66.2 & 47.6 & - \\
    %PointCNN & 85.9 & 63.9 & 57.3 & 88.1 & 75.6 & 65.4 & 45.8 \\
    %SPGraph & 86.4 & 66.5 & 58.0 & 85.5 & 73.0 & 62.1 & - \\
    %PointWeb & 87.0 & 66.6 & 60.3 & 87.3 & 76.2 & 66.7 & - \\
    MinkowskiNet~\cite{choy20194d} & - & 71.7 & 65.4 & - & - & - & 67.9 \\
    PointTransformer~\cite{zhao2021point}~\cite{qian2022pointnext}  & 90.8 & 76.5 & 70.4 & 90.2 & 81.9 & 73.5 & 70.6\\
    PointNeXt~\cite{qian2022pointnext} & 90.7 & - & 70.8 & 90.3 & - & 74.9 & 71.5 \\
    Stratified Trans~\cite{lai2022stratified} & 91.5 & 78.1 & 72.0 & - & - & - & 74.3\\
    PointMetaBase~\cite{lin2022meta} & 91.4 & - & 72.0 & 91.3 & - & 77.0 & 72.8\\
    SR-UNet~\cite{xie2020pointcontrast} & 89.1 & 75.5 & 68.2 & 90.2 & 82.1 & 73.6 & 72.2 \\
    \midrule
    Jigsaw & 82.8 & - & 52.1 & 84.4 & - & 56.6& - \\
    OcCo & 85.9 & - & 55.4 & 85.1 & - & 58.5 & - \\
    STRL & -  & - & - & 84.2 & - & 57.1 & -\\ 
    PointContrast  &  - & 77.0 & 70.9 & - & - & - & 74.1 \\ 
    DepthContrast & -  & - & 70.6 & - & - & - & 71.2\\ 
    SceneContext &  - & - & 72.2 & - & - & - & 73.8 \\ 
    \rowcolor{gray!20} MVNet & \textbf{91.7}(91.6) & \textbf{79.5}(79.3) & \textbf{73.6}(73.3) & \textbf{91.8}(91.7) & \textbf{86.3}(86.2) & \textbf{78.3}(78.1) & \textbf{75.6}(75.2)\\
    
    %\rowcolor{gray!20}\textit{ Improvement} & \textcolor[rgb]{0,0.6,0}{+2.6} & \textcolor[rgb]{0,0.6,0}{+4.1} & \textcolor[rgb]{0,0.6,0}{+5.4} & \textcolor[rgb]{0,0.6,0}{+1.6} & \textcolor[rgb]{0,0.6,0}{+4.2} & \textcolor[rgb]{0,0.6,0}{+4.7} & \textcolor[rgb]{0,0.6,0}{+3.4}\\
    \bottomrule
\end{tabular}
\caption{\small{\textbf{Semantic segmentation results on S3DIS (evaluation by 6-Fold or in Area 5) and ScanNet V2.} We show Overall Accuracy (OA), mean Accuracy (mAcc), and mean Intersection over Union~(mIoU). Methods in the second section are self-supervised pre-training approaches. MVNet shows the average results of 3 runs.}}
\label{tab:semseg}
\end{table*}

==> chapters/MVNet/tables/shape_task_backup.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \resizebox{1.\linewidth}{!}{  
    \footnotesize
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Method} & Dataset & \multicolumn{3}{c}{ScanObjectNN} & \multicolumn{2}{c}{ShapeNetPart} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-6} & OBJ-BG & OBJ-ONLY & PB-T50-RS & ins. mIoU & cls. mIoU \\
        \midrule
        Transformer$^{\dagger}$ ~\citep{yu2022point} & & 79.9 & 80.6 & 77.2 & 85.1 & 83.4 \\
        PointBERT~\citep{yu2022point} & & 87.4 & 88.1 & 83.1 & 85.6 & 84.1 \\
        MaskDiscr~\citep{Liu2022maskdis} & & 89.7 & 89.3 & 84.3 & 86.0 & 84.4 \\
        MaskSurfel~\citep{zhang2022masked} & & 91.2 & 89.2 & 85.7 & 86.1 & 84.4 \\
        ULIP~\citep{xue2023ulip} & 91.3 & & 89.4 & 86.4 & - & - \\
        PointMAE~\citep{pang2022masked} & & 90.0 & 88.3 & 85.2 & 86.1 & - \\
        \rowcolor{gray!20}MVNet-B & \textbf{91.5} & \textbf{90.1}  & \textbf{87.8} & \textbf{86.2} & \textbf{84.8} \\       
        \rowcolor{gray!20}MVNet-L & \textbf{95.2} & \textbf{94.2}  & \textbf{91.0} & \textbf{86.8} & \textbf{85.2} \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\footnotesize{\textbf{Performance comparison with other pre-training approaches on shape-level downstream tasks.} All the methods and MVNet-B use the same transformer backbone architecture. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
    \label{tab:shape-result}
    %\vspace{-3pt}
\end{table*}



==> chapters/MVNet/tables/supervised_seg.tex <==
\begin{table*}[h]
\centering
\scriptsize
\setlength\tabcolsep{4pt}
\begin{tabular}{llllllll}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{S3DIS Area 5} & \multicolumn{3}{c}{S3DIS 6-Fold} & ScanNet \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8} & OA & mAcc & mIoU & OA & mAcc & mIoU & mIoU \\
    \midrule
    PointNet~\citep{qi2017pointnet} & 53.5 & 49.0 & 41.1 & 78.5 & 66.2 & 47.6 & - \\
    PointCNN~\citep{li2018pointcnn} & 85.9 & 63.9 & 57.3 & 88.1 & 75.6 & 65.4 & 45.8 \\
    SPGraph~\citep{landrieu2018large} & 86.4 & 66.5 & 58.0 & 85.5 & 73.0 & 62.1 & - \\
    PointWeb~\citep{zhao2019pointweb} & 87.0 & 66.6 & 60.3 & 87.3 & 76.2 & 66.7 & - \\
    MinkowskiNet~\citep{choy20194d} & - & 71.7 & 65.4 & - & - & - & 67.9 \\
    Vision MVFusion~\citep{DBLP:conf/eccv/KunduYFRBFP20} & - & - & 65.4 & - & - & - & 74.6\\
    Voint Cloud~\citep{DBLP:conf/iclr/HamdiGG23} & - & - & 66.1 & - & - & - & 74.8 \\
    PointTransformer~\citep{zhao2021point}  & 90.8 & 76.5 & 70.4 & 90.2 & 81.9 & 73.5 & 70.6\\
    PointNeXt~\citep{qian2022pointnext} & 90.7 & - & 70.8 & 90.3 & - & 74.9 & 71.5 \\
    Stratified Trans~\citep{lai2022stratified} & 91.5 & 78.1 & 72.0 & - & - & - & 74.3\\
    PointMetaBase~\citep{lin2022meta} & 91.4 & - & 72.0 & 91.3 & - & 77.0 & 72.8\\
    SR-UNet~\citep{xie2020pointcontrast} & 89.1 & 75.5 & 68.2 & 90.2 & 82.1 & 73.6 & 72.2 \\
    \rowcolor{gray!20} MVNet & \textbf{91.7}(91.6) & \textbf{79.5}(79.3) & \textbf{73.8}(73.3) & \textbf{91.8}(91.7) & \textbf{86.3}(86.2) & \textbf{78.3}(78.1) & \textbf{75.6}(75.2)\\
    
    %\rowcolor{gray!20}\textit{ Improvement} & \textcolor[rgb]{0,0.6,0}{+2.6} & \textcolor[rgb]{0,0.6,0}{+4.1} & \textcolor[rgb]{0,0.6,0}{+5.4} & \textcolor[rgb]{0,0.6,0}{+1.6} & \textcolor[rgb]{0,0.6,0}{+4.2} & \textcolor[rgb]{0,0.6,0}{+4.7} & \textcolor[rgb]{0,0.6,0}{+3.4}\\
    \bottomrule
\end{tabular}
\caption{\small{\textbf{Comparison with supervised methods on S3DIS (evaluation by 6-Fold or in Area 5) and ScanNet V2.} The average result of 3 runs is given in parentheses.}}
\label{tab:supp-seg}
\end{table*}

==> chapters/MVNet/tables/supp_fewshot.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{8pt}% 调整列间距
\scriptsize

\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
\cmidrule(lr){2-3}   \cmidrule(lr){4-5}
 & 10-shot & 20-shot & 10-shot & 20-shot \\
\hline
DGCNN$^{\dagger}$ & $31.6 \pm 2.8$ & $40.8 \pm 4.6$ & $19.9 \pm 2.1$ & $16.9 \pm 1.5$ \\
OcCo & $90.6 \pm 2.8$ & $92.5 \pm 1.9$ & $82.9 \pm 1.3$ & $86.5 \pm 2.2$ \\
CrossPoint & $92.5 \pm 3.0$ & $94.9 \pm 2.1$ & $83.6 \pm 5.3$ & $87.9 \pm 4.2$ \\
\hline
Transformer$^{\dagger}$ & $87.8 \pm 5.2$ & $93.3 \pm 4.3$ & $84.6 \pm 5.5$ & $89.4 \pm 6.3$ \\
OcCo & $94.0 \pm 3.6$ & $95.9 \pm 2.3$ & $89.4 \pm 5.1$ & $92.4 \pm 4.6$ \\
PointBERT & $94.6 \pm 3.1$ & $96.3 \pm 2.7$ & $91.0 \pm 5.4$ & $92.7 \pm 5.1$ \\
MaskDiscr & $95.0 \pm 3.7$ & $97.2 \pm 1.7$ & $91.4 \pm 4.0$ & $93.4 \pm 3.5$ \\
PointMAE & $96.3 \pm 2.5$ & $97.8 \pm 1.8$ & $92.6 \pm 4.1$ & $95.0 \pm 3.0$ \\
\rowcolor{gray!20} MVNet & $\pmb{97.2} \pm \pmb{1.8}$ & $\pmb{98.3} \pm \pmb{1.8}$ &  $\pmb{93.4} \pm \pmb{3.4}$ & $\pmb{95.8} \pm \pmb{3.2}$ \\
\bottomrule
\end{tabular}
\caption{\small{\textbf{Few-shot classification on ModelNet40.} We report the average accuracy (\%) and standard deviation (\%) of 10 independent experiments. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
\label{tab:mn_fewshot}

\end{table*}

==> chapters/MVNet/tables/supp_label_eff.tex <==
\begin{table}[h]
\centering
\setlength\tabcolsep{8pt}
\begin{tabular}{lccc}
\toprule
\textbf{Method}            & \textbf{20\%} & \textbf{50\%} & \textbf{100\%} \\ 
\midrule
Train from scratch & 18.8          & 24.7          & 32.9           \\ 
PointContrast      & 24.5          & 29.2          & 37.5           \\ 
4DContrast         & 26.3          & 31.5          & 38.2           \\ 
MVNet              & \textbf{28.5} & \textbf{33.2} & \textbf{39.6}  \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Label efficient training on SUN RGB-D object detection task.} We take the VoteNet as network architecture and compare our method with PointContrast and 4DContrast.}
\label{tab:supp-label}
\end{table}


==> chapters/MVNet/tables/supp_shape_task.tex <==
\begin{table*}[t]
    \centering
    \resizebox{1.\linewidth}{!}{  
    \footnotesize
    \begin{tabular}{llccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c}{ScanObjectNN} & \multicolumn{2}{c}{ShapeNetPart} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-7} & & OBJ-BG & OBJ-ONLY & PB-T50-RS & ins. mIoU & cls. mIoU \\
        \midrule
        Jigsaw~\citep{sauder2019self} & DGCNN & 86.8 & 86.2 & 83.5 & 85.3 & - \\
        OcCo~\citep{wang2020unsupervised} & DGCNN & 88.2& 87.5 & 85.0 &  - \\
        CrossPoint~\citep{afham2022crosspoint} & DGCNN & - & - & 85.5 & 83.7\\
        ULIP~\citep{xue2023ulip} & Transformer & 91.3 & 89.4 & 86.4 & - & -\\
        ULIP~\citep{xue2023ulip} & PointMLP & 93.2 & 90.4 & 89.4 & - & -\\
        Point-M2AE~\citep{zhang2022point} & M2AE & 91.2 & 88.8 & 86.4 & 86.5 & 84.9\\
        I2P-MAE~\cite{zhang2023learning} & M2AE & 94.2 & 91.6 & 90.1 & \textbf{86.8} & \textbf{85.2}\\
        \rowcolor{gray!20}MVNet-L & Transformer & \textbf{95.2} & \textbf{94.2}  & \textbf{91.0} & \textbf{86.8} & \textbf{85.2} \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Performance comparison with pre-training approaches using different network backbones on shape-level downstream tasks.} }}
    \label{tab:supp-shape-result}
    %\vspace{-3pt}
\end{table*}



==> chapters/MaskFeat3D/Tables/augmentation.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{ccc|c}
        \toprule
        rotation & scaling & translation & ScanObjectNN \\ 
        \midrule
        $\surd$ & - & - & 87.0\\
        - & $\surd$ & - & 85.9\\
        $\surd$ & $\surd$ & - & \textbf{87.6}\\
        - & $\surd$ & $\surd$ & 85.1\\
        $\surd$ & $\surd$ & $\surd$ & 86.7 \\   
         
        \bottomrule
    \end{tabular}
    \captionof{table}{Ablation study on pretraining data augmentation.}
    \label{tab:aug}
\end{table}

==> chapters/MaskFeat3D/Tables/feature_ablation_2.tex <==
\begin{table}[t]
    \centering
    \setlength\tabcolsep{10pt}
    \resizebox{0.9\linewidth}{!}{  
    \scriptsize
    \begin{tabular}{llc}
        \toprule
      \textbf{Method}  & \textbf{Target Feature} & \textbf{ScanNN}\\
      \midrule
      \multirow{4}{*}{PointMAE}  & position only & 85.2 \\
        & position + normal$^*$ & 85.7 \\
        & position + surface variation$^*$ & 85.9 \\
        & position + normal + variation$^*$ & 86.0 \\
        \midrule
       \multirow{3}{*}{MaskFeat3D} & normal & 86.5 \\
        & surface variation & 87.0\\
         & normal + variation & \textbf{87.7}\\
        % \midrule
        % SDF value & 85.2 \\
        % SDF Gradient & 84.8 \\       
        \bottomrule
    \end{tabular}
    }
    % \vspace{2pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Ablation study on different features.} $^*$ uses position-index matching~\cite{zhang2022masked} for feature loss computation.}}
    %Normal and surface variation, which corresponds to first-order and second-order differential properties, are complementary to each other. Therefore, reconstructing them together yields salient performance gains from reconstructing one of them.}
    \label{tab:feature_ablation}
\end{table}

==> chapters/MaskFeat3D/Tables/fewshot_feat_ab.tex <==
\begin{table*}[t]

\begin{minipage}[b]{.55\linewidth}
\centering
\setlength\tabcolsep{4pt}% 调整列间距
\scriptsize

\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
\cmidrule(lr){2-3}   \cmidrule(lr){4-5}
 & 10-shot & 20-shot & 10-shot & 20-shot \\
\hline
DGCNN$^{\dagger}$ & $31.6 \pm 2.8$ & $40.8 \pm 4.6$ & $19.9 \pm 2.1$ & $16.9 \pm 1.5$ \\
OcCo & $90.6 \pm 2.8$ & $92.5 \pm 1.9$ & $82.9 \pm 1.3$ & $86.5 \pm 2.2$ \\
CrossPoint & $92.5 \pm 3.0$ & $94.9 \pm 2.1$ & $83.6 \pm 5.3$ & $87.9 \pm 4.2$ \\
\hline
Transformer$^{\dagger}$ & $87.8 \pm 5.2$ & $93.3 \pm 4.3$ & $84.6 \pm 5.5$ & $89.4 \pm 6.3$ \\
OcCo & $94.0 \pm 3.6$ & $95.9 \pm 2.3$ & $89.4 \pm 5.1$ & $92.4 \pm 4.6$ \\
PointBERT & $94.6 \pm 3.1$ & $96.3 \pm 2.7$ & $91.0 \pm 5.4$ & $92.7 \pm 5.1$ \\
MaskDiscr & $95.0 \pm 3.7$ & $97.2 \pm 1.7$ & $91.4 \pm 4.0$ & $93.4 \pm 3.5$ \\
PointMAE & $96.3 \pm 2.5$ & $97.8 \pm 1.8$ & $92.6 \pm 4.1$ & $95.0 \pm 3.0$ \\
\rowcolor{gray!20} MaskFeat3D & $\pmb{97.1} \pm \pmb{2.1}$ & $\pmb{98.4} \pm \pmb{1.6}$ &  $\pmb{93.4} \pm \pmb{3.8}$ & $\pmb{95.7} \pm \pmb{3.4}$ \\
\bottomrule
\end{tabular}
\caption{\small{\textbf{Few-shot classification on ModelNet40.} We report the average accuracy (\%) and standard deviation (\%) of 10 independent experiments.}}
\label{tab:mn_fewshot}
\end{minipage}\hspace{.01\linewidth}
\begin{minipage}[b]{.43\linewidth}
\scriptsize
\setlength\tabcolsep{4pt}

\begin{tabular}{llc}
        \toprule
      \textbf{Method}  & \textbf{Target Feature} & \textbf{ScanNN}\\
      \midrule
      \multirow{4}{*}{PointMAE}  & position only & 85.2 \\
        & position + normal$^*$ & 85.7 \\
        & position + surface variation$^*$ & 85.9 \\
        & position + normal + variation$^*$ & 86.0 \\
        \midrule
       \multirow{3}{*}{MaskFeat3D} & normal & 86.5 \\
        & surface variation & 87.0\\
         & normal + variation & \textbf{87.7}\\
        % \midrule
        % SDF value & 85.2 \\
        % SDF Gradient & 84.8 \\       
        \bottomrule
\end{tabular}

\captionof{table}{\small{\textbf{Ablation study on different features.} $^*$ uses position-index matching~\cite{zhang2022masked} for feature loss computation.}}
\label{tab:feature_ablation}
\end{minipage}
\end{table*}

==> chapters/MaskFeat3D/Tables/modelnet40_fewshot.tex <==
\begin{table}[t]
\centering
\setlength\tabcolsep{4pt}
\renewcommand\arraystretch{1}
%\small
\sisetup{
  table-align-uncertainty=true,
  separate-uncertainty=true,
}
%% local redefinitions
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
\fontsize{8pt}{11pt}\selectfont

\resizebox{1\linewidth}{!}{
    \scriptsize
\begin{tabular}{lcccc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
\cmidrule(lr){2-3}   \cmidrule(lr){4-5}
 & 10-shot & 20-shot & 10-shot & 20-shot \\
\hline
DGCNN$^{\dagger}$~\cite{dgcnn:2019:tog} & $31.6 \pm 2.8$ & $40.8 \pm 4.6$ & $19.9 \pm 2.1$ & $16.9 \pm 1.5$ \\
OcCo~\cite{wang2021unsupervised} & $90.6 \pm 2.8$ & $92.5 \pm 1.9$ & $82.9 \pm 1.3$ & $86.5 \pm 2.2$ \\
CrossPoint~\cite{afham2022crosspoint} & $92.5 \pm 3.0$ & $94.9 \pm 2.1$ & $83.6 \pm 5.3$ & $87.9 \pm 4.2$ \\
\hline
Transformer$^{\dagger}$~\cite{Yu_2022_CVPR} & $87.8 \pm 5.2$ & $93.3 \pm 4.3$ & $84.6 \pm 5.5$ & $89.4 \pm 6.3$ \\
OcCo~\cite{wang2021unsupervised} & $94.0 \pm 3.6$ & $95.9 \pm 2.3$ & $89.4 \pm 5.1$ & $92.4 \pm 4.6$ \\
PointBERT~\cite{Yu_2022_CVPR} & $94.6 \pm 3.1$ & $96.3 \pm 2.7$ & $91.0 \pm 5.4$ & $92.7 \pm 5.1$ \\
MaskDiscr~\cite{Liu2022maskdis} & $95.0 \pm 3.7$ & $97.2 \pm 1.7$ & $91.4 \pm 4.0$ & $93.4 \pm 3.5$ \\
PointMAE~\cite{Pang2022MaskedAF} & $96.3 \pm 2.5$ & $97.8 \pm 1.8$ & $92.6 \pm 4.1$ & $95.0 \pm 3.0$ \\
\rowcolor{gray!20} MaskFeat3D & $\pmb{97.1} \pm \pmb{2.1}$ & $\pmb{98.4} \pm \pmb{1.6}$ &  $\pmb{93.4} \pm \pmb{3.8}$ & $\pmb{95.7} \pm \pmb{3.4}$ \\
\bottomrule
\end{tabular}
}
\label{tab:mn_fewshot}
\vspace{-2mm}
\caption{\small{\textbf{Few-shot classification on ModelNet40.} We report the average accuracy (\%) and standard deviation (\%) of 10 independent experiments.}}
%\vspace{-2mm}
\end{table}

==> chapters/MaskFeat3D/Tables/modelnet40_finetune.tex <==
\begin{table}[t]
    \centering

    %
    %\footnotesize
    \begin{tabular}{lc}
        \toprule
        \textbf{Method} & \textbf{ModelNet40} \\
        \midrule
        Transformer$^{\dagger}$ ~\cite{Yu_2022_CVPR}     & 91.4 \\
        PointBERT~\cite{Yu_2022_CVPR}    & 93.2 \\
        MaskDiscr~\cite{Liu2022maskdis}  & 93.8 \\
        MaskSurfel~\cite{zhang2022masked} & 93.6 \\
        PointMAE~\cite{Pang2022MaskedAF} & 93.8 \\
        \rowcolor{gray!20}MaskFeat3D    & \textbf{93.9} \\
        \bottomrule
    \end{tabular}
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Shape classification fine-tuned on ModelNet40.} All the methods use the same transformer backbone architecture. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
    \label{tab:modelnet40}
    %\vspace{-3pt}
\end{table}



==> chapters/MaskFeat3D/Tables/pointnext_ablation.tex <==
\begin{wraptable}[19]{r}{0.56\linewidth}
    \centering
    \footnotesize
    \setlength\tabcolsep{3pt}
    \begin{tabular}{lccc}
        \toprule
       \textbf{cases} &  \textbf{channel}(c) & \textbf{ScanObjectNN} & \textbf{ShapeNetPart}\\
       \midrule
      \small{Scratch} & 3 & 87.1 & 85.6\\
      \small{MaskFeat3D} & 3 & 88.0 & 86.8\\
      \midrule
      \small{Scratch} & 4 & 88.1 & 86.0 \\
      \small{MaskFeat3D} & 4 & \textbf{88.6} & 87.0 \\
      \midrule
      \small{Scratch} & 7 & - & 87.1\\
      \small{MaskFeat3D} & 7 & - & \textbf{87.4}\\
        \bottomrule
    \end{tabular}
    \captionof{table}{\textbf{Comparison of PointNeXt backbone under different input channel numbers.}    `Scratch' means training from scratch. `MaskFeat3D' means fine-tuning on the pretrained weight of our model. We report overall accuracy for ScanObjectNN PB-T50-RS split, and ins. mIoU for ShapeNetPart task. Channel $c = 3$ means only using position. $c = 4$ uses position and height information. $c = 7$ uses position, height, and point normal. Since ScanObjectNN dataset does not contain point normal labels, we leave $c = 7$ entries blank.}
    \label{tab:pointnext_ablation} 
\end{wraptable}

==> chapters/MaskFeat3D/Tables/s3dis_2.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Sem Seg}}& \multicolumn{2}{c}{\textbf{Detection}} \\ 
      \cmidrule(lr){2-3}   \cmidrule(lr){4-5} &  mIoU & OA & mAP$_{0.25}$ & mAP$_{0.5}$ \\
        \midrule
        PointNet~\cite{qi2017pointnet} & 41.1 & 49.0 &  - & - \\ 
        PointNet++~\cite{qi2017pointnet++} & 53.5 & 67.1 & 46.1 & 24.5 \\
        PointCNN~\cite{pointcnn} & 57.3 & 85.9 &  - & - \\
        GSDN~\cite{gwak2020generative} & - & - & 47.8 & 25.1 \\
        DGCNN~\cite{dgcnn:2019:tog} & 47.9 & 83.6 & - & - \\
        PointTrans~\cite{pointr} & 70.4 & 90.8 &  - & - \\
        FCAF3D~\cite{rukhovich2022fcaf3d} & 65.4 & 89.1 & 66.7 & 45.9 \\
        PointNeXt~\cite{PointNeXt} & 70.8 & 90.7 &  - & - \\
        \midrule
        Point-MAE & 60.8 & 69.9 & - & - \\
        Point-M2AE~\cite{zhang2022point} & - & - & 50.1 & 33.2 \\
        \rowcolor{gray!20}MaskFeat3D & \textbf{71.7} & \textbf{91.7} & \textbf{71.6} & \textbf{49.2} \\
        \bottomrule
    \end{tabular}
    \vspace{2pt}
    \caption{\small{\textbf{Area 5 Semantic segmentation and detection results on S3DIS.}}}
    \label{tab:s3dis} 
    %\vspace{-4mm}
\end{table}



==> chapters/MaskFeat3D/Tables/s3dis_3.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Sem Seg}}& \multicolumn{2}{c}{\textbf{Detection}} \\ 
      \cmidrule(lr){2-3}   \cmidrule(lr){4-5} &  mIoU & OA & mAP$_{0.25}$ & mAP$_{0.5}$ \\
        %\midrule
        %PointNet~\cite{qi2017pointnet} & 41.1 & 49.0 &  - & - \\ 
        %PointNet++~\cite{qi2017pointnet++} & 53.5 & 67.1 & 46.1 & 24.5 \\
        %PointCNN~\cite{pointcnn} & 57.3 & 85.9 &  - & - \\
        %GSDN~\cite{gwak2020generative} & - & - & 47.8 & 25.1 \\
        %DGCNN~\cite{dgcnn:2019:tog} & 47.9 & 83.6 & - & - \\
       % PointTrans~\cite{pointr} & 70.4 & 90.8 &  - & - \\
        %Point-MAE & 60.8 & 69.9 & - & - \\
        %Point-M2AE~\cite{zhang2022point} & - & - & 50.1 & 33.2 \\
        \midrule
        PointNeXt$^{\dagger}$~\cite{PointNeXt} & 70.8 & 90.7 &  - & - \\
        MaskFeat3D & \textbf{71.7} & \textbf{91.7} & - & - \\
        \midrule
        FCAF3D$^{\dagger}$~\cite{rukhovich2022fcaf3d} & - & - & 66.7 & 45.9 \\
        MaskFeat3D & - & - & \textbf{71.6} & \textbf{49.2} \\
        \bottomrule
    \end{tabular}
    %\vspace{2pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Area 5 Semantic segmentation and detection results on S3DIS.} $^{\dagger}$ represents the \textit{from scratch} results and MaskFeat3D in the same section represents the \textit{fine-tuning} results using pretrained weights under same backbone.}}
    \label{tab:s3dis} 
    \vspace{-6mm}
\end{table}



==> chapters/MaskFeat3D/Tables/shape_segmentation.tex <==
\begin{table}
    \centering
    %\setlength\tabcolsep{20pt}
    \begin{tabular}{l|ll}
        \toprule
        \textbf{Method} & ins. mIoU & cls. mIoU\\
        \midrule
         PointNet & 83.7 & 80.4\\
        DGCNN & 85.2 & 82.3\\
        PointNet++ & 85.1 & 81.9\\
        PointTransform & 86.6 & 83.7\\
        PointMLP & 86.1 & 84.6 \\
        Stratified & 86.6 & 85.1 \\
        \midrule
        %Jigsaw\citep{sauder2019self} & 92.4\% \\
        
        PointViT & 85.1 & 83.4 \\
        $\text{[S]}$Point-BERT & 85.6 & 84.1\\
        $\text{[S]}$MaskPoint & 86.0 & 84.4 \\
        $\text{[S]}$Point-MAE & 86.1 & - \\
        \rowcolor{gray!20}$\text{[S]}$ MaskFeat & \textbf{86.2} $\pm$ 0.0\textcolor[rgb]{0,0.6,0}{(+0.1)}& \textbf{84.6} $\pm$ 0.1\textcolor[rgb]{0,0.6,0}{(+0.3)} \\
        \midrule
        MinkowskiNet & - & -\\
        \rowcolor{gray!20}$\text{[S]}$ MaskFeat & - & -\\
        \midrule
        PointNeXt & 87.0 $\pm$ 0.1 & 85.2 $\pm$ 0.1\\
        \rowcolor{gray!20}$\text{[S]}$ MaskFeat & \textbf{87.3} $\pm$ 0.1\textcolor[rgb]{0,0.6,0}{(+0.3)} & \textbf{85.3} $\pm$ 0.1 \textcolor[rgb]{0,0.6,0}{(+0.1)}\\
        \bottomrule
    \end{tabular}
    \captionof{table}{ShapeNetPart Segmentation.}
    \label{tab:sbnn}
\end{table}

==> chapters/MaskFeat3D/Tables/supp_ablation.tex <==
\begin{table*}[t]
%\scriptsize
\setlength\tabcolsep{10pt}
\begin{subtable}[t]{.3\textwidth}
\centering  
%\scriptsize
\footnotesize
\caption{\footnotesize \textbf{Neighborhood size}}
    \begin{tabular}{cc}
    \toprule
     r & ScanObjectNN \\
        \midrule
        0.05 & 86.6 \\
        0.07 & 87.0 \\
        \rowcolor{gray!20} 0.1 & \textbf{87.7} \\
        0.2 & 86.8 \\
        \bottomrule
    \end{tabular}
     \label{tab:sv_ablation}
\end{subtable}
 %\hfill
 \hspace*{0.017\textwidth}
\begin{subtable}[t]{.3\textwidth}
\centering  
%\scriptsize
\footnotesize
\caption{\footnotesize \textbf{Number $k$ in FPS}} 
\begin{tabular}{cc}
\toprule
        \# $k$ & ScanObjectNN \\ 
        \midrule
        8 & 87.4 \\
        16 & 87.4 \\
        \rowcolor{gray!20} 32 & \textbf{87.7} \\
        64 & 87.6 \\
        128 & 87.6 \\
        \bottomrule
    \end{tabular}
    \label{tab:fps}
\end{subtable}
 %\hfill 
\begin{subtable}[t]{.33\textwidth}
\centering  
\footnotesize
\caption{\footnotesize \textbf{Mask region}} 
    \begin{tabular}{cc}
    \toprule
     region & ScanObjectNN \\
        \midrule
        \rowcolor{gray!20} masked only & \textbf{87.7} \\
        all points & 86.8 \\
        \bottomrule
    \end{tabular}
    \label{tab:unmasked}
\end{subtable}

\caption{\small{\textbf{More ablation studies of our design choices}. Please refer to \cref{sec:supp-ablation} for more details.}}
\label{tab:ablation} \vspace{-5mm}
\end{table*}


==> chapters/MaskFeat3D/Tables/supp_fps.tex <==
\begin{table}[h]
    \centering
    %\footnotesize
    \vspace{-7pt}
    \scriptsize
    \begin{tabular}{cccccc}
        %\toprule
        \# $k$ & 8 & 16 & 32 & 64 & 128 \\
        \midrule
        ScanObjectNN & 87.4 & 87.4 & \textbf{87.7} & 87.6 & 87.6 \\
        %\bottomrule
    \end{tabular}
    %\caption{}
    \vspace{-12pt}
    \label{tab:fps} 
\end{table}



==> chapters/MaskFeat3D/Tables/supp_unmasked.tex <==
\begin{table}[h]
    \centering
    \scriptsize
    %\footnotesize
    \vspace{-8pt}
    \begin{tabular}{ccc}
        %\toprule
         & \textbf{masked only} & \textbf{all points} \\
        \midrule
        ScanObjectNN (PB-T50-RS) & \textbf{87.7} & 86.8 \\
        %\bottomrule
    \end{tabular}
    %\caption{}
    \vspace{-12pt}
    \label{tab:supp-unmask}
    
\end{table}



==> chapters/MaskFeat3D/Tables/sv_ablation.tex <==
\begin{table}
    \centering
    \begin{tabular}{cc}
    \toprule
     \textbf{r} & \textbf{ScanObjectNN} (OA(\%)) \\
        \midrule
        0.05 & 86.6 \\
        0.07 & 87.0 \\
        \rowcolor{gray!20} 0.1 & 87.7 \\
        0.2 & 86.8 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study on the neighborhood size} $r$ in shape surface variation. We utilize the ViT-based encoder and present the overall accuracy on the ScanObjectNN PB-T50-RS split.}
    \label{tab:sv_ablation}
\end{table}

==> chapters/MaskFeat3D/Tables/svm.tex <==
\begin{table}
    \centering
    \setlength\tabcolsep{20pt} 
    \resizebox{1.\linewidth}{!}{
    \footnotesize
    \begin{tabular}{lc}
        \toprule
        \textbf{Method} & \textbf{Acc. (\%)} \\
        \midrule
        %Random &  60.2\% \\
        3D-GAN~\cite{wu2016learning}  & 83.3 \\
        Latent-GAN~\cite{achlioptas2018learning} & 85.7 \\
        SO-Net~\cite{li2018so} & 87.3 \\
        MAP-VAE~\cite{han2019multi} & 88.4 \\
        Jigsaw~\cite{sauder2019self} & 84.1 \\
        FoldingNet~\cite{yang2018foldingnet} & 88.4 \\
        DGCNN + OcCo~\cite{wang2021unsupervised} & 89.7 \\
        DGCNN + STRL~\cite{huang2021spatio} & 90.9 \\
        DGCNN + IAE~\cite{yan2022implicit} & 92.1 \\
        Point-M2AE~\cite{zhang2022point} & \underline{92.9} \\
        \midrule 
        Transformer + OcCo$^*$~\cite{wang2021unsupervised} & 89.6 \\
        PointBERT~\cite{Yu_2022_CVPR}$^*$ & 87.4 \\
        %MaskDiscr$^*$ & \\
        PointMAE~\cite{Pang2022MaskedAF}$^*$ & 88.5 \\
        \rowcolor{gray!20}MaskFeat3D$^*$ & \textbf{91.1}\\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Linear evaluation for shape classification on ModelNet40}. This task is sensitive to the encoder backbone. Different * methods use the same Transformer encoder backbone.}} 
    \vspace{-2mm}
    \label{tab:svm}
\end{table}

==> chapters/acknowledgement.tex <==
\begin{acknowledgments}		% Optional
\index{Acknowledgments@\emph{Acknowledgments}}%


My Ph.D. dissertation would not be possible without the incredible support of many people. First and foremost, I would like to express my deepest gratitude to my Ph.D. advisor, Prof. Qixing Huang. In my heart, Qixing’s passion and dedication to research have been truly inspiring. Throughout my Ph.D. journey, he has taught me not only how to be a researcher but also how to explore new fields from the ground up. His keen insights and commitment to deep, valuable research have profoundly influenced me.
I feel incredibly fortunate to have been Qixing’s student. This five-year journey has been an invaluable experience in my life. I will carry the lessons he taught me and strive to embody the qualities of a dedicated researcher in my future endeavors.

I also want to thank my committee members Prof. Qiang Liu, Georgios Pavlakos, and Gang Hua for providing me with valuable feedback on my dissertation. I am especially grateful to Prof. Gang Hua. I was an intern in his team at Wormpex in the summer of 2020. Despite being very busy, he always found time to mentor me in detail together with Haoxiang Li during my internship. In every meeting, Gang could quickly identify the key issues in my research. We together conducted wonderful research and produced a well-formulated paper.
Furthermore, he offered me tremendous support in my job search and career advice after the internship, always willing to help whenever I needed it. It was a great honor to be his intern, and I am deeply thankful for his guidance and support.

I also want to express my gratitude to Dr. Yang Liu and Xin Tong from my Microsoft internship. Dr. Liu always understood what I wanted to express during our discussions, and I learned a great deal from him. Dr. Tong had a remarkable ability to grasp the key issues in our current research and guide me in the right direction.
And I want to thank Erran Li, Min Bai, Weifeng Chen, and Xiong Zhou from my Amazon internship. Erran and Min helped me explore a completely new direction in my research, and I was deeply impressed by their guidance and support during the internship.

I also want to thank Chongyang Ma, Haibin Huang, Yue Wang, Xinshuo Wen during my summer internship at Kuaishou and Nvidia. Both internships are impressive and I learnt a lot. And I want to thank my lab-mates Zhenpei Yang, Chen Song, Haitao Yang, Bo Sun, Zaiwei Zhang, Yifan Sun, Xiangru Huang, Jiaxin Lu, Hanwen Jiang, Zhenxiao Liang, Zihang He, Yuezhi Yang for their fruitful discussions. I'd also want to thank all my paper collaborators for their input. 
I especially want to thank Chen Song, Haitao Yang, and Bo Sun. We joined the group at the same time, all freshmen who knew very little initially. Over the past five years, we have shared many experiences together. We endured the challenging times of the COVID pandemic, and only we truly understand how difficult it was. Five years is a long time, and I feel incredibly fortunate to have had these three wonderful friends by my side throughout my Ph.D. journey.

I want to thank my family back in China. I have not been able to back home for many years, but I can constantly feel their love and support surrounding me.
Finally, I want to extend my deepest thanks to my girlfriend. Over the past five years, we have lived in different countries and time zones, making it incredibly challenging to maintain our relationship. Despite these obstacles, she has provided me with immense support, and I am certain that I could not have successfully completed this journey without her by my side. 


\end{acknowledgments}
